DiffPortrait360: Consistent Portrait Diffusion for 360 View Synthesis

Generating high-quality 360-degree views of human heads from single-view images is essential for enabling accessible immersive telepresence applications and scalable personalized content creation. While cutting-edge methods for full head generation are limited to modeling realistic human heads, the latest diffusion-based approaches for style-omniscient head synthesis can produce only frontal views and struggle with view consistency, preventing their conversion into true 3D models for rendering from arbitrary angles. We introduce a novel approach that generates fully consistent 360-degree head views, accommodating human, stylized, and anthropomorphic forms, including accessories like glasses and hats. Our method builds on the DiffPortrait3D framework, incorporating a custom ControlNet for back-of-head detail generation and a dual appearance module to ensure global front-back consistency. By training on continuous view sequences and integrating a back reference image, our approach achieves robust, locally continuous view synthesis. Our model can be used to produce high-quality neural radiance fields (NeRFs) for real-time, free-viewpoint rendering, outperforming state-of-the-art methods in object synthesis and 360-degree head generation for very challenging input portraits.

==> figures/failure_cases.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.97\linewidth]{example-image-a}
	\centering
        \vspace{-3mm}
	\caption[Caption for LOF]{\textbf{Failure cases.} }  % expression, pose, appearance.
    \label{fig:failure}
\end{figure}

==> figures/supply/more_ablation_consis.tex <==
\begin{figure*}%[htbp]% 
\centering
\includegraphics[width=1.0\linewidth]{example-image-golden}
\caption{More visual results for the ablation study on view-consistency control.}
\label{fig:ablation_consis_more}
\end{figure*}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Reconstructing a full 3D appearance of the head from a single unconstrained portrait image has been a longstanding challenge in computer vision. In this work, we introduce a tailored diffusion-based generative network that produces consistent 360-degree novel view images from a single unrestricted input image. This method addresses the significant style and view consistency variations that typically occur with large viewing angles. Even with limited training data, it maintains strong style generalization capabilities. To the best of our knowledge, this is the first  \textit{inference-based} zero-shot approach that enables view-consistent, \textit{high-fidelity full-head} portrait image synthesis renderable in \textit{360$^{\circ}$}. Beyond preserving consistency, our method naturally supports stylized images across various non-facial domains and can generate a full-head view from a single extreme side view image.

Typically, long-range portrait view synthesis from sparse inputs requires a generative prior to hallucinate plausible scene features that are not observed in the inputs. Recently, 3D-Aware Generative Adversarial Networks (GANs) have advanced rapidly, driven by the integration of implicit neural representations for 3D scene modeling with style-based generative networks for image synthesis. The pioneering 3D GAN, EG3D\cite{Chan2022}, has demonstrated impressive quality in view-consistent image synthesis. However, despite achieving high-quality novel view synthesis, limitations in its representation, such as the triplane\cite{Chan2022} structure, introduce strong projection ambiguities for 360-degree camera poses. Additionally, back-view camera poses are challenging to obtain, limiting the model’s focus to near-front faces.

To address large view-angle changes, follow-up research has explored new representations for reconstructing 360-degree head views, often without constrained data or accurate back-view camera poses. These approaches aim to capture a wider range of hairstyles and full-head details. However, 3D-aware GAN methods \cite{An_2023_CVPR, li2024spherehead} trained on limited datasets, even with new representations, struggle to faithfully depict 360-degree 3D faces. This often results in a loss of resemblance, distorted geometry, or blurred extrapolation Figure \ref{fig:compare_real}.

With the recent rise of large-scale text-to-image diffusion models, such as Imagen\cite{saharia2022photorealistic} and Stable Diffusion\cite{rombach2022high}, we have seen unprecedented diversity and stability in image synthesis. Motivated by this progress, we aim to leverage the generative capabilities of these production-ready diffusion models for full-head 360-degree novel view synthesis. Unlike previous 3D-aware GAN methods, which attempt to invert a reference image into generative noise or a textual description, these methods face challenges in consistently translating the image into a 3D scene. Such approaches struggle to retain appearance consistency when the generated view deviates significantly from the reference view.

Recently, the diffusion-based 3D-aware synthesis method, DiffPortrait3D\cite{Gu_2024_CVPR}, approached this problem using a controlled Stable Diffusion framework (specifically SD1.5). It cross-queries appearance context from the source image through self-attention layers in the Stable Diffusion U-Net, with camera views controlled by explicitly rendered 3DGAN images enhanced with cross-attention. However, limited appearance control in DiffPortrait3D restricts it from achieving true full-head 360-degree synthesis. We argue that the stability of novel view appearances is strongly correlated with the degree of overlap between the input appearance and the newly generated view; when this overlap is minimal, the appearance content cannot be consistently preserved Figure \ref{fig:ablation}.

In this work, we introduce Diffportrait360, a novel zero-shot framework that utilizes a 2D diffusion model to synthesize 360-degree 3D consistent novel views from a single portrait. Given just one portrait image, Diffportrai360 demonstrates the ability to generate reasonable and consistent novel views, even under large camera view changes (far from the near face), and exhibits robust generalization capabilities, remaining unaffected by variations in camera alignment or the style of the input image. Building on prior 3D-aware novel view synthesis works, such as Diffportrait3D, we have developed a dual appearance module to address the challenges associated with 360-degree view changes from the input image, specifically the entanglement of content and spatial consistency. We argue that the stability of novel view appearances is strongly correlated with the degree of overlap between the input appearance and the new view angle. When this overlap is minimal, it becomes difficult to ensure the consistency of the appearance content. Additionally, the lack of extensive stylized data for the back of the head, if trained only on real data, would result in a significant bias in the data distribution for back-view stylization Figure\ref{fig:ablation_back}. To address this issue, we have compiled a dataset of stylized images to scale up and enhance our content stylization consistency, effectively overcoming the bias in real dataset for the back of the head. The consistency is further strengthened by our novel consistent training strategy.

We have conducted extensive evaluations of DiffPortrait360 on our challenging benchmarks, demonstrating its universal effectiveness for generating consistent 360-degree views of out-of-domain portraits without any fine-tuning. Our method exceeds the performance of state-of-the-art full-head novel view synthesis baselines, achieving superior visual quality, resemblance, and view consistency both quantitatively and qualitatively. 

The contributions of our work can be summarized as follows:

\begin{itemize}
\item We present a novel $360^\circ$ view synthesis method from a single style-omniscient portrait that extends pre-trained stable diffusion models with consistent appearance control.

\item A stable diffusion-based back view generator paired with a dual appearance control module that enables the synthesis of globally consistent views around the subject.

\item A novel training strategy that suggests the use of view consistent sequence generation to promote continuity and smoothness, combined with a 3D head datasets consisting of captured and synthetic subjects.

\end{itemize}
Our code and model will be available for research purposes. 
